The Population Posterior and Bayesian Inference on Streams

Many modern data analysis problems involve inferences from streaming data. However, streaming data is not easily amenable to the standard probabilistic modeling approaches, which assume that we condition on finite data. We develop population variational Bayes, a new approach for using Bayesian modeling to analyze streams of data. It approximates a new type of distribution, the population posterior, which combines the notion of a population distribution of the data with Bayesian inference in a probabilistic model. We study our method with latent Dirichlet allocation and Dirichlet process mixtures on several large-scale data sets.

==> preamble.tex <==
\usepackage[T1]{fontenc}
\renewcommand*\ttdefault{lmvtt}

%% USE THIS IF YOU DON'T HAVE MTPRO2
\usepackage{mathptmx}
\usepackage{amsmath}
\usepackage{amsthm}
\usepackage{amssymb}


%% USE THIS IF YOU HAVE MTPRO2
% \usepackage{tgtermes}
% \usepackage[subscriptcorrection,slantedGreek,nofontinfo,mtpbb,mtpcal,amssymbols]{mtpro2}
% \usepackage{scalefnt,letltxmacro}
% \LetLtxMacro{\oldtextsc}{\textsc}
% \renewcommand{\textsc}[1]{\oldtextsc{\scalefont{1.25}#1}}

% ADDITIONAL PACKAGES (remove if anything causes trouble)
\usepackage[final,expansion=alltext]{microtype}     % fixes some LaTeX weirdness
\usepackage{graphicx}                               % graphics
\usepackage{amsmath}                                % math
\usepackage[labelfont=bf]{caption}                  % bold figure/table label
\usepackage[format=hang]{subcaption}                % subfigures
\usepackage{booktabs}                               % nice tables
%\usepackage[algoruled]{algorithm2e}                 % pseudocode
\usepackage[numbers,sort]{natbib}                   % better bibliography
\usepackage{cleveref}                               % the best package ever
\usepackage[acronym,smallcaps,nowarn]{glossaries}   % second best package ever

% \usepackage{tikz}
% \usetikzlibrary{external}\tikzexternalize

% \usepackage{pgfplots,pgfplotstable}
% \usepgfplotslibrary{fillbetween}
% \pgfplotsset{compat=newest}
% \pgfplotsset{plot coordinates/math parser=false}
% \usepgfplotslibrary{colorbrewer}                    % <-MUST INSTALL SEPARATELY!
% \newlength\figureheight
% \newlength\figurewidth
% \setlength\figureheight{2.0in}
% \setlength\figurewidth{2.75in}

% HELPER FUNCTIONS
\DeclareRobustCommand{\parhead}[1]{\textbf{#1} }
\DeclareRobustCommand{\PP}{{\sffamily\color{purple}\P{}} }
\renewcommand\bibsection{\subsubsection*{\refname}} % make References section
                                                    % header match NIPS

\crefname{equation}{eq.}{eqs.}
\Crefname{equation}{Eq.}{Eqs.}
\creflabelformat{equation}{#2#1#3}

